Compositional Generalization in Image Captioning

Image captioning models are usually evaluated on their ability to describe a held-out set of images, not on their ability to generalize to unseen concepts. We study the problem of compositional generalization, which measures how well a model composes unseen combinations of concepts when describing images. State-of-the-art image captioning models show poor generalization performance on this task. We propose a multi-task model to address the poor performance, that combines caption generation and image--sentence ranking, and uses a decoding mechanism that re-ranks the captions according their similarity to the image. This model is substantially better at generalizing to unseen combinations of concepts compared to state-of-the-art captioning models.

==> diversity.tex <==
\section{Diversity in Generated Captions}\label{appendix:diversity}

Table \ref{tab:diversity} shows the diversity scores for \textsc{butd} and \modelname{} as well as for the top-scoring models taken from \citet{van2018measuring}.

\begin{table*}[ht]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Model & ASL & SDSL & Types & TTR$_1$ & TTR$_2$ & \%Novel & Cov & Loc$_5$ \\ \midrule
\citet{liu2017mat} & \textbf{10.3} & 1.32 & 598 & 0.17 &  0.38 & 50.1 & 0.05 & 0.70 \\
\citet{vinyals2017show} & 10.1 & 1.28 & 953 & 0.21 & 0.43 & 90.5 & 0.07 & 0.69 \\
\citet{shetty2017speaking} &  9.4 & 1.31 & \textbf{2611} & 0.24 & 0.54 & 80.5 & \textbf{0.20} & 0.71 \\
\textsc{butd} & 9.0 & 1.01 & 1162 & 0.22 & 0.49 & 56.4 & 0.09 & 0.78 \\
\modelname & 10.2 & \textbf{1.76} & 1882 & \textbf{0.26} & \textbf{0.59} & \textbf{93.6} & 0.14 & \textbf{0.80} \\ 
\midrule
Validation data & 11.3 & 2.61 & 9200 & 0.32 & 0.72 & 95.3 & - & - \\
\bottomrule
\end{tabular}
\caption[Scores for diversity metrics as defined by \citet{van2018measuring} for different models.]{\label{tab:diversity} Scores for diversity metrics as defined by \citet{van2018measuring} for different models. Scores for \textsc{butr} and \modelname{} are calculated on the COCO validation set, scores for all other models and the validation data (last row) are taken from \citet{van2018measuring}.}
\end{table*}

